Measurement of the branching fractions of the singly Cabibbo-suppressed decays $\Lambda_{c}^{+}\to p\eta$ and $\Lambda_{c}^{+}\to p\omega$

Based on 4.5 $\mbox{fb$^{-1}$}$ $e^{+}e^{-}$ collision data collected with BESIII detector at seven energy points between 4.600 and 4.699 GeV, the branching fractions for $\Lambda_{c}^{+}\to p\eta$ and $\Lambda_{c}^{+}\to p\omega$ were measured by means of single-tag method. The branching fractions of $\Lambda_{c}^{+}\to p\eta$ and $\Lambda_{c}^{+}\to p\omega$ are determined to be $(1.57\pm0.11_{\rm {stat}}\pm0.04_{\rm{syst}})\times10^{-3}$ and $(1.11\pm0.20_{\rm{stat}}\pm0.07_{\rm{syst}})\times10^{-3}$, with a statistical significance of greater than 10 $\sigma$ and 5.7 $\sigma$, respectively. These results are consistent with the previous measurements by BESIII, LHCb and Belle, and the result of $\Lambda_{c}^{+}\to p\eta$ is the most precise to date.

==> feynman.tex <==
\begin{figure}[!tbp]
\centering
%==================================================================
    \hspace{-15mm}
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(u\)};
				\vertex[right=3cm of a1] (a2) {\(u\)};
		
				\vertex[below=2em of a1] (b1) {\(d\)};
				\vertex[right=3cm of b1] (b2) {\(d\)};
		
				\vertex[below=4em of b1] (c1) {\(c\)};
				\vertex[right=1cm of c1] (c2);
				\vertex[below=4em of b2] (c3) {\(d\)};
		
				\vertex[above=1.5em of c3] (d1) {\(\overline d\)};
				\vertex[above=1em of d1] (d3) {\(u\)};
				\vertex at ($(d1)!0.5!(d3) - (1cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2),
						(b1) -- (b2),
						(c1) -- (c2) -- (c3),
					},
					(d1) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d3),
					(c2) -- [boson, bend left, edge label=\(W^{\pm}\)] (d2),
				};
		
				\draw [decoration={brace}, decorate] (a2.east) -- (d3.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d1.east) -- (c3.east) node  [pos=0.5, right] {\(\eta\)/\omega};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		%\captionsetup{justification=centering}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman1}
		\vspace{5mm}
	\end{subfigure}
	\hspace{10mm}
%==================================================================
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(u\)};
				\vertex[right=3cm of a1] (a2) {\(u\)};
		
				\vertex[below=2em of a1] (b1) {\(d\)};
				\vertex[right=3cm of b1] (b2) {\(d\)};
		
				\vertex[below=4em of b1] (c1) {\(c\)};
				\vertex[right=1cm of c1] (c2);
				\vertex[below=4em of b2] (c3) {\(s\)};
		
				\vertex[above=1.5em of c3] (d1) {\(\overline s\)};
				\vertex[above=1em of d1] (d3) {\(u\)};
				\vertex at ($(d1)!0.5!(d3) - (1cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2),
						(b1) -- (b2),
						(c1) -- (c2) -- (c3),
					},
					(d1) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d3),
					(c2) -- [boson, bend left, edge label=\(W^{\pm}\)] (d2),
				};
		
				\draw [decoration={brace}, decorate] (a2.east) -- (d3.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d1.east) -- (c3.east) node  [pos=0.5, right] {\(\eta\)};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman2}
		\vspace{5mm}
	\end{subfigure}
	\hspace{10mm}
%==================================================================
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(u\)};
				\vertex[right=3cm of a1] (a2) {\(u\)};
		
				\vertex[below=2em of a1] (b1) {\(c\)};
				\vertex[right=1cm of b1] (b2);
				\vertex[below=2em of a2] (b3) {\(d\)};
		
				\vertex[below=4em of b1] (c1) {\(d\)};
				\vertex[right=3cm of c1] (c2) {\(d\)};
		
				\vertex[below=1.5em of b3] (d1) {\(u\)};
				\vertex[below=1em of d1] (d3) {\(\overline d\)};
				\vertex at ($(d3)!0.5!(d1) - (1cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2),
						(b1) -- (b2) -- (b3),
						(c1) -- (c2),
					},
					(d3) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d1),
					(d2) -- [boson, bend left, edge label=\(W^{\pm}\)] (b2),
				};
		
				\draw [decoration={brace}, decorate] (a2.east) -- (d1.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d3.east) -- (c2.east) node  [pos=0.5, right] {\(\eta\)/\omega};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman3}
		\vspace{5mm}
	\end{subfigure}
	
%==================================================================
    \hspace{-15mm}
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(u\)};
				\vertex[right=3cm of a1] (a2) {\(u\)};
				
				\vertex[below=2em of a1] (b1) {\(d\)};
				\vertex[right=1.2cm of b1] (b2);
				\vertex[below=2em of a2] (b3) {\(u\)};
				
				\vertex[below=4em of b1] (c1) {\(c\)};
				\vertex[right=1.2cm of c1] (c2);
				\vertex[below=4em of b3] (c3) {\(d\)};
				
				\vertex[below=1.3em of b3] (d1) {\(d\)};
				\vertex[below=1.4em of d1] (d3) {\(\overline d\)};
				\vertex at ($(d1)!0.5!(d3) - (1.5cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2),
						(b1) -- (b2) -- (b3),
						(c1) -- (c2) -- (c3),
					},
					(d3) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d1),
					(c2) -- [boson, edge label=\(W^{\pm}\)] (b2),
				};
		
				\draw [decoration={brace}, decorate] (a2.east) -- (d1.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d3.east) -- (c3.east) node  [pos=0.5, right] {\(\eta\)/\omega};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman4}
	\end{subfigure}
	\hspace{10mm}
%==================================================================
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(u\)};
				\vertex[right=3cm of a1] (a2) {\(u\)};
		
				\vertex[below=2em of a1] (b1) {\(c\)};
				\vertex[right=1.2cm of b1] (b2);
				\vertex[below=2em of a2] (b3) {\(d\)};
		
				\vertex[below=4em of b1] (c1) {\(d\)};
				\vertex[right=1.2cm of c1] (c2);
				\vertex[below=4em of b3] (c3) {\(u\)};
		
				\vertex[below=1.3em of b3] (d1) {\(u\)};
				\vertex[below=1.4em of d1] (d3) {\(\overline u\)};
				\vertex at ($(d1)!0.5!(d3) - (1.5cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2),
						(b1) -- (b2) -- (b3),
						(c1) -- (c2) -- (c3),
					},
					(d3) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d1),
					(c2) -- [boson, edge label=\(W^{\pm}\)] (b2),
				};
		
				\draw [decoration={brace}, decorate] (a2.east) -- (d1.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d3.east) -- (c3.east) node  [pos=0.5, right] {\(\eta\)/\omega};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman5}
	\end{subfigure}
	\hspace{10mm}
%==================================================================
	\begin{subfigure}[t]{0.25\linewidth}
		\begin{tikzpicture}
			\begin{feynman}
				\vertex(a1){\(d\)};
				\vertex[right=1.2cm of a1] (a2);
				\vertex[right=1.8cm of a2] (a3) {\(u\)};
		
				\vertex[below=2em of a1] (b1) {\(c\)};
				\vertex[right=1.2cm of b1] (b2);
				\vertex[below=2em of a3] (b3) {\(d\)};
		
				\vertex[below=4em of b1] (c1) {\(u\)};
				\vertex[below=4em of b3] (c2) {\(u\)};
		
				\vertex[below=1.3em of b3] (d1) {\(u\)};
				\vertex[below=1.4em of d1] (d3) {\(\overline u\)};
				\vertex at ($(d1)!0.5!(d3) - (1.5cm, 0)$) (d2);
		
				\diagram* {
					{[edges=fermion]
						(a1) -- (a2) -- (a3),
						(b1) -- (b2) -- (b3),
						(c1) -- (c2),
					},
					(d3) -- [fermion, out=180, in=-45](d2) -- [fermion, out=45, in=180] (d1),
					(a2) -- [boson, edge label=\(W^{\pm}\)] (b2),
				};
		
				\draw [decoration={brace}, decorate] (a3.east) -- (d1.east) node  [pos=0.5, right] {\(p\)};
				\draw [decoration={brace}, decorate] (d3.east) -- (c2.east) node  [pos=0.5, right] {\(\eta\)/\omega};
				\draw [decoration={brace}, decorate] (c1.west) -- (a1.west) node  [pos=0.5, left] {\(\Lambda_{c}^{+}\)};
			\end{feynman}
		\end{tikzpicture}
		\captionsetup{margin={35pt, 0pt}}
		\caption{}
		\label{fig:feynman6}
	\end{subfigure}
%==================================================================
	\caption{Feynman diagrams for $\Lambda_{c}^{+}\rightarrow p\eta/\omega$. Plots (a), (b) and (c) correspond to internal W-emission diagrams, while plots (d), (e) and (f) are W-exchange diagrams.}
	\label{fig:feynman}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	

